Decoupled Strategy for Imbalanced Workloads in MapReduce Frameworks

In this work, we consider the integration of MPI one-sided communication and non-blocking I/O in HPC-centric MapReduce frameworks. Using a decoupled strategy, we aim to overlap the Map and Reduce phases of the algorithm by allowing processes to communicate and synchronize using solely one-sided operations. Hence, we effectively increase the performance in situations where the workload per process is unexpectedly unbalanced. Using a Word-Count implementation and a large dataset from the Purdue MapReduce Benchmarks Suite (PUMA), we demonstrate that our approach can provide up to 23% performance improvement on average compared to a reference MapReduce implementation that uses state-of-the-art MPI collective communication and I/O.

==> Makefile <==

all: main.pdf

main.pdf: main.tex
	@pdflatex main.tex -interaction nonstopmode 2>&1 1>main.pdf.log
	@- bibtex main.aux 2>&1 1>main.pdf.log
	@pdflatex main.tex -interaction nonstopmode 2>&1 1>main.pdf.log
	@pdflatex main.tex -interaction nonstopmode 2>&1 1>main.pdf.log
	@while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log 2> /dev/null) do pdflatex main.tex -interaction nonstopmode 2>&1 1>main.pdf.log; done 2>&1 1>main.pdf.log

acmart.cls: acmart.ins
	latex acmart.ins

clean:
	@$(RM) *.log *.aux *.pdf \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

rebuild: clean all


